Repaint123: Fast and High-quality One Image to 3D Generation with Progressive Controllable 2D Repainting

Recent one image to 3D generation methods commonly adopt Score Distillation Sampling (SDS). Despite the impressive results, there are multiple deficiencies including multi-view inconsistency, over-saturated and over-smoothed textures, as well as the slow generation speed. To address these deficiencies, we present Repaint123 to alleviate multi-view bias as well as texture degradation and speed up the generation process. The core idea is to combine the powerful image generation capability of the 2D diffusion model and the texture alignment ability of the repainting strategy for generating high-quality multi-view images with consistency. We further propose visibility-aware adaptive repainting strength for overlap regions to enhance the generated image quality in the repainting process. The generated high-quality and multi-view consistent images enable the use of simple Mean Square Error (MSE) loss for fast 3D content generation. We conduct extensive experiments and show that our method has a superior ability to generate high-quality 3D content with multi-view consistency and fine textures in 2 minutes from scratch. Our project page is available at https://pku-yuangroup.github.io/repaint123/.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{fig/motivation.png}
    \caption{Motivation of our proposed pipeline. Current methods adopt SDS loss (causing oversaturation and inconsistency) or multistep MSE loss (extremely slow). We propose to progressively repaint unseen regions from the reference view to all views, controlled by coarse geometry and reference fine texture. This enables }
    \label{fig:motivation}
\end{figure}

The generation of 3D content from one image occupies a key role at the intersection of computer vision and computer graphics[], serving as a pivotal conduit for innovative applications across robotics, virtual reality, and augmented reality. Nonetheless, the task of generating multi-view consistent 3D objects from a singular view continues to pose a substantial challenge, mainly due to the lack of 3D information contained in a single image. 


The advent of the diffusion model[] has notably propelled 2D image generation, with some studies further incorporating spatial conditioning, such as depth maps, for controllable generation. It has also catalyzed progress in 3D generation, where numerous works employ Score Distillation Sampling (SDS) loss to directly distill the prior knowledge of 2D image diffusion models into 3D constructs. Despite their remarkable outcomes in semantic and geometric generation, three prevalent challenges persist: over-saturation, over-smoothness owing to nondeterministic optimization, and sluggish optimization due to extensive diffusion reverse pass at each step.

Several studies[] attempt to mitigate oversaturation through multistep Mean Squared Error (MSE) loss, but challenges of over-smoothness and slowness remain unresolved. Alternate works fine-tune a 3D diffusion model for accelerated multi-view image generation and reconstruction. However, due to training on limited and synthetic multi-view datasets, the generated images exhibit view inconsistencies and suboptimal quality compared to the real reference image, compromising both geometry and texture.


%\subsection{Our method}
To address texture inconsistencies and accelerate the optimization process during the refine stage, in this paper, we introduce a novel approach Repaint123 aimed at achieving high-fidelity and fast 3D generation from a single viewpoint. The core idea involves viewing the generation of new perspectives as a diffusion process of textures based on reference view, which create textures for other novel views incrementally, starting with the reference view. Specifically, We project the depth map onto the point cloud using the existing geometry from the coarse stage in order to determine the occlusion areas in relation to the previously refined views, and repaint the texture of the occlusion areas using 2D diffusion and the geometric priors. In order to maintain long-term consistency and improve the overall harmony of the 3D object's texture, we also suggest a mutual self-attention technique and the image prompts to stop accumulation of texture deviations brought by the repaint process. 

We conduct thorough experiments using 2D pictures from multiple datasets. The extensive experiments show that our method is able to generate high-quality and view-consistent 3D objects more efficiently. It takes about 
 \textbf{2 } minutes to train from scratch and obtain a high-quality, 3D object %if using faster Gaussian Splatting[] at the coarse stage. 
%Also, as a plug-and-play pipeline, our approach is highly generalizable and can be applied to the refine stage of text-3d tasks.
when compared to state-of-the-art techniques, Our methodology represents a major step towards more high-quality 3D generation, significantly improving view consistency, visual quality and speed.


In summary, our work has the following contributions:
\begin{itemize}

\item Repaint123 comprehensively considers controllable repainting process for single-view 3D generation, containing both geometry prior and long short-term texture prior. 
%It has achieved a leading level of visual quality and reconstruction speed among current single-view generation methods.

\item We propose a progressive refinement pipeline with visibility-aware adaptive repainting masks. This enables view-consistent high-quality 3D generation for about \textbf{2} minutes.

% \item Our method, as a plug-and-play module, is robust to different 3D representations and generation tasks. Using Gaussian Splatting in the coarse stage, we reconstruct high-quality 3D model from single-view image in less than 5 minutes.
\item  Through a comprehensive series of experiments, our method has consistently demonstrated exceptional generation fidelity within minimal optimization time.

\end{itemize}


%\subsection{Dual submission}

%Please refer to the author guidelines on the \confName\ \confYear\ web page for a
%discussion of the policy on dual submissions.

%\subsection{Paper length}
%Papers, excluding the references section, must be no longer than eight pages in length.
%The references section will not be included in the page count, and there is no limit on the length of the references section.
%For example, a paper of eight pages with two pages of references would have %a total length of 10 pages.
%{\bf There will be no extra page charges for \confName\ \confYear.}

%verlength papers will simply not be reviewed.
%This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
%Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
%The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
%The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

%Reviewers:
%note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
%Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


%\subsection{Paper ID}
%Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
%If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


%\subsection{Mathematics}

%examples:
%\begin{equation}
%  E = m\cdot c^2
%  \label{eq:important}
%\end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/1_intro_pyt.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{fig/motivation.pdf}
    \caption{Motivation of our proposed pipeline. Current methods adopt SDS loss, resulting in oversaturation and inconsistency. We propose to progressively repaint unseen regions from the reference view to all views, controlled by coarse geometry and reference fine texture. This enables }
    \label{fig:motivation}
\end{figure}

The generation of 3D content from one image plays a key role at the intersection of computer vision and computer graphics~\cite{liu2023zero123,liu2023syncdreamer,jun2023shap,nichol2022point,qian2023magic123,dou2023tore}, serving as a pivotal conduit for innovative applications across fields including robotics, virtual reality, and augmented reality. Nonetheless, this task is quite challenging since it is expected to generate multi-view consistent and high-quality 3D content in a short time.

%  主要思路： 吹我们的方法，速度又快，texture又好， view consistent; 分别对应 gussian + mse, repaint ，long term control. 而别的方法无法这么全能。
Recent studies utilize diffusion models~\cite{diffusion1,diffusion2}, which have notably advanced image generation techniques, to assist 3D generation from text or image by distilling their prior knowledge via Score Distillation Sampling (SDS)~\cite{dreamfusion}. Despite their remarkable outcomes, \textit{\textbf{three challenges}} are widely acknowledged, including view-inconsistency from different perspectives, limited quality with over-saturated and over-smoothed generated texture, and cumbersome optimization due to extensive reverse diffusion steps. To continuously improve the 3D generation techniques, several studies attempt to address the above-mentioned challenges with different focuses. 
To improve multi-view consistency, some works~\cite{shi2023mvdream,long2023wonder3d} fine-tune a multi-view diffusion model to generate view-consistent images for further 3D reconstruction. However, due to limited and synthetic multi-view datasets that are used for training, the generated images from the multi-view diffusion model may demonstrate view inconsistency and sub-optimal quality, resulting in low-quality 3D content. 
Aiming to improve generation quality, some works~\cite{qian2023magic123,weng2023consistent123} incorporate 2D diffusion with textual inversion~\cite{gal2022textualinversion} as guidance for generation. Although generation quality is improved, there exists inconsistency within the generated 3D novel views per se, as well as with the reference view. These works are also extremely slow as textual inversion needs hours for optimization.
In order to speed up the generation process, some works~\cite{tang2023dreamgaussian,yi2023gaussiandreamer} propose the utilization of a novel 3D Gaussian Splatting~\cite{kerbl2023gaussiansplatting} as a representation; however, the texture quality is significantly compromised. Some ohter works train a model to generate 3D representation such as point cloud~\cite{nichol2022point} and implicit function~\cite{jun2023shap}. Although the generation process is fast, the generated 3D contents are of low quality compared to SDS optimization-based methods.

%\subsection{Our method}
To address these three deficiencies mentioned above, we propose a novel method called Repaint123 for fast and high-quality 3D content generation from a single image. As shown in Figure \ref{fig:motivation}, our method adopts a two-stage optimization strategy. The first stage follows DreamGaussian~\cite{tang2023dreamgaussian} to obtain a coarsely painted 3D model in 1 minute. In the second stage, the core idea involves progressively repainting the occlusion areas controlled by the geometry prior from the coarse 3D model and appearance priors of the coarse texture and the reference image. Specifically, for consistent multi-view image generation, we ensure low-frequency 3D-consistent color information preservation by deterministic inversion and ensure neighbor consistency by repainting the 3D model progressively with accurate alignment in the overlaps and harmony between overlaps and near occlusions. To alleviate accumulated texture deviations and ensure long-term texture consistency, we adopt a mutual self-attention strategy to inject attention features of the reference image into the novel-view diffusion denoising process. Constrained by the long short-term consistency, we can improve the 3D model quality by enhancing the quality of the generated multi-view images. For enhanced image quality, we propose a normal-based repainting to refine the overlap regions with different strengths based on the previous best visibility on these regions. Besides, we use a pre-trained 2D diffusion model with the reference image as an image prompt to perform classifier-free guidance for high-quality image generation. For speed, with the fast splatting-optimized 3D model and fast high-quality consistent multi-view images, we can do fast sparse-view reconstruction of the 3D content using MSE loss.


% For multi-view consistent image generation, we   As shown in Figure \ref{fig:motivation}, 

We conduct thorough experiments using 2D images from multiple datasets. The extensive experiments show that our method is able to generate high-quality and view-consistent 3D objects efficiently. It takes about 
 \textbf{2 minutes} to generate a high-quality 3D object from scratch.%if using faster Gaussian Splatting[] at the coarse stage. 
%Also, as a plug-and-play pipeline, our approach is highly generalizable and can be applied to the refine stage of text-3d tasks.
Compared to state-of-the-art techniques, our method represents a major step towards high-quality 3D generation, significantly improving view consistency, visual quality, and generation speed.


In summary, our work has the following contributions:
\begin{itemize}

\item Repaint123 comprehensively considers controllable repainting process for single-view 3D generation, containing both geometry prior and long short-term texture prior. 
%It has achieved a leading level of visual quality and reconstruction speed among current single-view generation methods.

\item We propose a two-stage optimization-based pipeline for fast single-view 3D generation. With a Splatting-based coarse stage and a fast progressive refinement pipeline, we can generate view-consistent high-quality 3D content for about \textbf{2} minutes.

% \item Our method, as a plug-and-play module, is robust to different 3D representations and generation tasks. Using Gaussian Splatting in the coarse stage, we reconstruct high-quality 3D model from single-view image in less than 5 minutes.
\item  Through a comprehensive series of experiments, our method has consistently demonstrated exceptional generation quality within minimal optimization time. 

\end{itemize}


%\subsection{Dual submission}

%Please refer to the author guidelines on the \confName\ \confYear\ web page for a
%discussion of the policy on dual submissions.

%\subsection{Paper length}
%Papers, excluding the references section, must be no longer than eight pages in length.
%The references section will not be included in the page count, and there is no limit on the length of the references section.
%For example, a paper of eight pages with two pages of references would have %a total length of 10 pages.
%{\bf There will be no extra page charges for \confName\ \confYear.}

%verlength papers will simply not be reviewed.
%This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
%Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
%The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
%The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

%Reviewers:
%note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
%Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


%\subsection{Paper ID}
%Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
%If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


%\subsection{Mathematics}

%examples:
%\begin{equation}
%  E = m\cdot c^2
%  \label{eq:important}
%\end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> tables/ablation_angle.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering

\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{c|ccccc}
\toprule \textbf{Metrics\textbackslash{}Angles}
 & \textit{20}  & \textit{30} & \textit{40} & \textit{50} & \textit{60}  \\ \midrule
CLIP-similarity$\uparrow$ & 0.58  & 0.61  & 0.87  & 0.61  & 0.58  \\
LPIPS$\downarrow$         & 0.04  & 0.04  & 1.38  & 0.06  & 0.08  \\ 
PSNR$\uparrow$           & 23.96 & 24.05 & 29.38 & 23.75 & 23.34 \\
LPIPS$\downarrow$         & 0.04  & 0.04  & 0.012  & 0.06  & 0.08  \\ \bottomrule
\end{tabular}%
}
\caption{Effects of the chosen angle of neighboring viewpoints in Repaint123 on Test-alpha dataset.}
\label{tab:ablate_2d_3d}
\end{table}

==> tables/sota.tex <==
% \begin{table*}[h]
% \centering
% \caption{\textbf{Repaint123 results.} We show quantitative results in terms of CLIP-Similarity$\uparrow$ / Contextual-Distance$\downarrow$ / PSNR$\uparrow$ / LPIPS$\downarrow$. The results are shown on the Realfusion15 and test-alpha datasets, while \textbf{bold} reflects the best.}
% \label{table:Image-to-3D}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}c|cccccccc@{}}
% \toprule
% \textbf{Dataset} & \textbf{Metrics\textbackslash{}Methods} 
% & RealFusion 
% & Zero-1-to-3 &Make-It-3D & Magic123 & \textbf{Repaint123} (\textbf{Ours})\\
% \midrule
% \multirow{4}{*}{\textbf{RealFusion15}} 
% & CLIP-Similarity$\uparrow$ & 0.67 & 0.75 &  
%  & 0.80 &\textbf{0.84} \\ 
% & Contextual-Distance$\downarrow$&  &  &  & 1.60 & \textbf{1.53} \\
% & PSNR$\uparrow$  &0.67 & 19.49 & & 19.13 & \textbf{19.48} \\
% & LPIPS$\downarrow$  & 0.14 & 0.11 &   &0.10 &\textbf{0.09} \\ 
% \midrule
% \multirow{4}{*}{\textbf{Test-alpha}}        
% & CLIP-Similarity$\uparrow$  & &  &  &0.84  & \textbf{0.87} \\
% & Contextual-Distance$\downarrow$  &  & &  & 1.48 & \textbf{1.38} \\
% & PSNR$\uparrow$       &  &  &  & 29.04 & \textbf{29.38} \\
% & LPIPS$\downarrow$    &  &  &  & \textbf{0.010} & 0.012\\ 

% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{figure}[h] 
\centering
\includegraphics[width=\textwidth]{fig/sota.pdf}
% \vspace{1em}
% \includegraphics[width=\textwidth]{figures/src/sota-nerf4.pdf}
\caption{
{Qualitative comparisons on image-to-3D generation.
}
\label{fig:sota1}
\end{figure}

% \begin{table}[t]
% \centering
% \caption{Quantitative results in terms of CLIP-Similarity$\uparrow$ / PSNR$\uparrow$ / LPIPS$\downarrow$. \textbf{Bold} reflects the best.}
% \label{table:Image-to-3D}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Dataset} & Point-E~\cite{PointE} & Shap-E~\cite{ShapeE} 
% & 3DFuse~\cite{3DFuse} & NeuralLift~\cite{NeuralLift}  & RealFusion~\cite{RealFusion}
% & Zero-1-to-3~\cite{Zero-1-to-3} & \textbf{Magic123} (\textbf{Ours}) \\
% \midrule
% NeRF4 & 0.48 / 0.70 / 0.80 & 0.60 / 0.99 / 0.76 & 0.60 / 5.86 / 0.76 & 0.52 / 12.55 / 0.50 & 0.38 / 15.37 / 0.20& 0.62 / 23.96 / 0.05 & \textbf{0.80 / 24.76 / 0.03}
% \\
% RealFusion15 & 0.53 / 0.98 / 0.78 & 0.59 / 1.23 / 0.74 & 
% 0.67 / 6.28 / 0.80 & 0.65 / 11.08 / 0.53 & 0.67 / 18.87 / 0.14 & 0.75 / 19.49 / 0.11 & \textbf{0.81 / 19.63 / 0.09} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}
